On The Impact of Machine Learning Randomness on Group Fairness

Statistical measures for group fairness in machine learning reflect the gap in performance of algorithms across different groups. These measures, however, exhibit a high variance between different training instances, which makes them unreliable for empirical evaluation of fairness. What causes this high variance? We investigate the impact on group fairness of different sources of randomness in training neural networks. We show that the variance in group fairness measures is rooted in the high volatility of the learning process on under-represented groups. Further, we recognize the dominant source of randomness as the stochasticity of data order during training. Based on these findings, we show how one can control group-level accuracy (i.e., model fairness), with high efficiency and negligible impact on the model's overall performance, by simply changing the data order for a single epoch.

==> sections/sec_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Variance in Fair Machine Learning}
There has been a growing awareness of high variance in fair deep learning, associated with non-determinism in model training or underlying implementation \cite{amir2021impact,sellam2021multiberts,soares2022your,qian2021my}, and the uncertainty of existing results in literature.

Soares et al. \cite{soares2022your} investigate the relationship between various algorithmic choices and the corresponding fairness variance, in large language models. They study correlation of fairness with model size and found no obvious trends, as opposed to various claims previously made in literature \cite{bender2021dangers,hooker2020characterising}. They also found that fairness is heavily affected by the random seed, i.e. simply changing the random seed in the same setting can cause huge variance in fairness.

Sellam et al. \cite{sellam2021multiberts} have trained and released 25 pre-trained BERT checkpoints for the community, each trained from scratch with a different random seed. They also analyze the variance of model fairness and the impact of commonly used bias mitigation algorithms on downstream tasks when starting with different pre-trained models, They show that while bias mitigation is capable of improving fairness scores on downstream tasks on average, there is significant variance across changing random seeds to question the value of such mitigation techniques.

Amir et al. \cite{amir2021impact} revisit state-of-the-art bias mitigation in-processing techniques in clinical texts and show a lack of statistically significant improvement after accounting for non-determinism in training. 
While existing literature focuses on exploring the impact of fairness variance in bias evaluation, we instead focus on investigating the source of this non-determinism. Furthermore, we propose to move away from the practise of simply executing multiple training runs to capture this variance and instead provide a computationally efficient proxy.

\subsection{Data Order and Example Forgetting}

Controlling the data order during training has gained noticeable success in improving convergence speeds in neural network training \cite{bengio2009curriculum,shah2020choosing,soviany2022curriculum,mohtashami2022characterizing}, while its adversarial capabilities have also been explored \cite{shumailov2021manipulating}.
Even under randomly shuffled data order, neural networks are known to undergo changes in predictive behavior during training \cite{toneva2018empirical,kirkpatrick2017overcoming,jagielski2022measuring,tirumala2022memorization}. We extend the discussion on non-determinism in model behavior to model fairness, and investigate its connections with data order.
We focus specifically on the instability in predictions made by the learning model and not its internal state, as we are concerned about the disparity in group level decisions which highlights the encoded bias.

==> sections/sec_reproducibility.tex <==
\section{Reproducibility Statement}
Our work studies various sources of non-determinism in neural model training and its impact on model fairness. Thus, it is important to address the implementation choices we have made to allow easy reproducibility. We provide a minimal psuedo code in Appendix \ref{sec:app_non_determinism} to clearly define various random seeds used in our setup to control training non-determinism. The complete training and evaluation pipeline is deterministic outside the choice of these random seeds, i.e., one can perfectly replicate the training by simply fixing these seeds. We will release our code to allow easy adaptation for future research.

==> slides/slides_preamble.tex <==

\usetheme{metropolis}
\usepackage{appendixnumberbeamer}


\usepackage{booktabs}
\usepackage[scale=2]{ccicons}
\usepackage{comment}


\usepackage{media9}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{dateplot}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}
\usetikzlibrary{arrows,automata}
\usetikzlibrary{positioning,calc,hobby}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{decorations.pathreplacing}

\usepackage{xspace}
\newcommand{\themename}{\textbf{\textsc{metropolis}}\xspace}

\setbeamersize{text margin left=5mm,text margin right=5mm} 

%my packages
\usepackage{multicol}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{tikz-layers}
\usepackage{relsize}
\usepackage{hyperref}
\usetikzlibrary{positioning}
\usepackage[makeroom]{cancel}
\usepackage{mathtools}
\usepackage[percent]{overpic}
\usepackage{algorithm}
\usepackage{algpseudocodex}
\usepackage{ulem}
\usepackage{cancel}
\usepackage{bbm}
\usepackage{transparent}

\bibliographystyle{apalike}
\newcommand{\citet}[1]{\cite{#1}}
%\usepackage{lmodern}
\usepackage[english]{babel}
\usefonttheme{professionalfonts}
\usepackage{exscale}
\usepackage{transparent}

\usepackage{bbm}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\suplog}{sup\,log}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\conv}{\text{conv}}
\newcommand{\COMPAS}{COMPAS }


\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\delert}[1]{\textcolor{gray}{#1}} % opposite of alert

\mode<presentation> { \setbeamercovered{transparent} }
\setbeamertemplate{navigation symbols}{}
\makeatletter
\def\beamerorig@set@color{%
	\pdfliteral{\current@color}%
	\aftergroup\reset@color
}
\def\beamerorig@reset@color{\pdfliteral{\current@color}}

\newcommand{\norm}[2]{\left\lVert#1\right\rVert_{#2}}

%\begin{tikzpicture}[overlay]
%	\node at (10,4.0){    \includegraphics[width=.175\textwidth]{adversary.PNG}};
%\end{tikzpicture}

\title{On The Impact of Machine Learning Randomness on Group Fairness}
\author{\textbf{Prakhar Ganesh}, Hongyan Chang, Martin Strobel, Reza Shokri}

%\institute{NUS Computing}
\date{FAccT 2023}
\titlegraphic{\includegraphics[height=1cm]{images/NUS.png}}

\defbeamertemplate{footnote}{unnumbered}{%
	\usebeamercolor[fg]{framesource}%
	\usebeamerfont{framesource}%
	\hfill\insertfootnotetext%
}

\newcommand{\source}[1]{%
	\setbeamertemplate{footnote}[unnumbered]%
	\footnotetext{Source: #1}%
}

%colors from https://www.r-bloggers.com/2013/02/the-paul-tol-21-color-salute/ (which are kind of taken in the original metropolis scheme)
%tol21rainbow= c("#771155", "#AA4488", "#CC99BB", "#114477", "#4477AA", "#77AADD", "#117777", "#44AAAA", "#77CCCC", "#117744", "#44AA77", "#88CCAA", "#777711", "#AAAA44", "#DDDD77", "#774411", "#AA7744", "#DDAA77", "#771122", "#AA4455", "#DD7788")

\definecolor{mTolDarkPurple}{HTML}{771155}
\definecolor{mTolPurple}{HTML}{AA4488}
\definecolor{mTolLightPurple}{HTML}{CC99BB}

\definecolor{mTolDarkBlue}{HTML}{114477}
\definecolor{mTolBlue}{HTML}{4477AA}
\definecolor{mTolLightBlue}{HTML}{77AADD}

\definecolor{mTolDarkTeal}{HTML}{117777}
\definecolor{mTolTeal}{HTML}{44AAAA}
\definecolor{mTolLightTeal}{HTML}{77CCCC}

\definecolor{mTolDarkGreen}{HTML}{117744}
\definecolor{mTolGreen}{HTML}{44AA77}
\definecolor{mTolLightGreen}{HTML}{88CCAA}

\definecolor{mTolDarkYellow}{HTML}{777711}
\definecolor{mTolYellow}{HTML}{AAAA44}
\definecolor{mTolLightYellow}{HTML}{DDDD77}

\definecolor{mTolDarkBrown}{HTML}{774411}
\definecolor{mTolBrown}{HTML}{AA7744}
\definecolor{mTolLightBrown}{HTML}{DDAA77}

\definecolor{mTolDarkRed}{HTML}{771122}
\definecolor{mTolRed}{HTML}{AA4455}
\definecolor{mTolLightRed}{HTML}{DD7788}


\pgfdeclareplotmark{check}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{cross}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{circle}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/circle.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkteal}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_teal.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossteal}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_teal.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkbrown}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_brown.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossbrown}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_brown.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkgreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_green.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossgreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_green.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkorange}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_orange.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossorange}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_orange.png}}(\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{circleorange}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/circle_orange.png}} (\pgfplotmarksize,\pgfplotmarksize);}


\pgfdeclareplotmark{checkmTolDarkPurple}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolDarkPurple.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkmTolPurple}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolPurple.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkmTolLightPurple}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolLightPurple.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{checkmTolDarkBrown}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolDarkBrown.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkmTolLightBrown}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolLightBrown.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{checkmTolDarkBlue}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolDarkBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkmTolBlue}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkmTolLightBlue}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolLightBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{checkmTolDarkGreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolDarkGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkmTolGreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]  	 {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{checkmTolLightGreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/check_mTolLightGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{crossmTolDarkBlue}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolDarkBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolBlue}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightBlue}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolLightBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{crossmTolDarkGreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolDarkGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolGreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]  	 {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightGreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolLightGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{crossmTolDarkPurple}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolDarkPurple.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightPurple}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolLightPurple.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{crossmTolDarkBrown}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolDarkBrown.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightBrown}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/cross_mTolLightBrown.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{circlemTolDarkGreen}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/circle_mTolDarkGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{circlemTolLightBlue}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/circle_mTolLightBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{circlemTolLightPurple}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/circle_mTolLightPurple.png}} (\pgfplotmarksize,\pgfplotmarksize);}




\pgfdeclareplotmark{circlemTolDarkGreen15}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/circle_mTolDarkGreen15.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolDarkGreen15}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/cross_mTolDarkGreen15.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{circlemTolLightBlue15}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/circle_mTolLightBlue15.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightBlue15}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/cross_mTolLightBlue15.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{circlemTolDarkGreen30}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/circle_mTolDarkGreen30.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolDarkGreen30}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/cross_mTolDarkGreen30.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{circlemTolLightBlue30}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/circle_mTolLightBlue30.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightBlue30}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/cross_mTolLightBlue30.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{circlemTolDarkGreen70}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/circle_mTolDarkGreen70.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolDarkGreen70}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/cross_mTolDarkGreen70.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{circlemTolLightBlue70}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/circle_mTolLightBlue70.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightBlue70}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/opacity/cross_mTolLightBlue70.png}} (\pgfplotmarksize,\pgfplotmarksize);}


\pgfdeclareplotmark{circlemTolDarkGreenHighlight}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/highlight/circle_mTolDarkGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{circlemTolLightBlueHighlight}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/highlight/circle_mTolLightBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfdeclareplotmark{crossmTolDarkGreenHighlight}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/highlight/cross_mTolDarkGreen.png}} (\pgfplotmarksize,\pgfplotmarksize);}
\pgfdeclareplotmark{crossmTolLightBlueHighlight}
{\path[opacity=0] (-\pgfplotmarksize,-\pgfplotmarksize) -- node[opacity=1]   {\includegraphics[width=2\pgfplotmarksize]{images/highlight/cross_mTolLightBlue.png}} (\pgfplotmarksize,\pgfplotmarksize);}

\pgfplotsset{
	discard if not/.style 2 args={
		x filter/.code={
			\edef\tempa{\thisrow{#1}}
			\edef\tempb{#2}
			\ifx\tempa\tempb
			\else
			\def\pgfmathresult{inf}
			\fi
		}
	}
}

\makeatletter
\pgfplotstableset{
	discard if not/.style 2 args={
		row predicate/.code={
			\def\pgfplotstable@loc@TMPd{\pgfplotstablegetelem{##1}{#1}\of}
			\expandafter\pgfplotstable@loc@TMPd\pgfplotstablename
			\edef\tempa{\pgfplotsretval}
			\edef\tempb{#2}
			\ifx\tempa\tempb
			\else
			\pgfplotstableuserowfalse
			\fi
		}
	}
}
\makeatother

\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        only marks,
        mark=-,
        mark size=1em,
        /pgfplots/error bars/.cd,
        y dir=plus,
        y explicit,
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw[ thick]  ##1 -- ++(1em,0pt) |- ##2 -- ++(-1em,0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=2,
        y error expr={\thisrowno{3}-\thisrowno{2}},
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path[ thick] ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=4,
        y error expr={\thisrowno{2}-\thisrowno{4}},
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path[ thick] ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=5,
        y error expr={\thisrowno{3}-\thisrowno{5}},
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot
    }
}


\definecolor{blue}{RGB}{31,120,180}
\definecolor{bblue}{RGB}{166,206,227}
\definecolor{green}{RGB}{ 251,154,153}
\definecolor{red}{RGB}{51,160,44}
\definecolor{bred}{RGB}{178,223,138} 
\setbeamercolor{palette martin}{%
  use=normal text,
  fg= blue,
  bg= bblue
}
\setbeamercolor{frametitle}{%
  use=palette martin,
  parent=palette martin
}
